Causal Theories of Relativistic Hydrodynamics

The first-order textbook formulations of relativistic viscous hydrodynamics are unstable and acausal. These shortcomings may be rectified by using effective theories which maintain stability and causality. In this dissertation, which is intended to also serve as an introduction to the field, causal theories of relativistic hydrodynamics are developed and explored. Conditions are obtained for a linearized analysis to predict the non-linear causality of a theory, and constraints are found on short-wavelength dispersion relations as a consequence of ensuring stability in all reference frames. First-order causal theories of hydrodynamics are extracted from kinetic theory and holography descriptions. Finally, causal theories describing charged plasmas (one-form magnetohydrodynamics), and describing superfluids are developed.

==> macros/initial_commands.tex <==
% These commands are used
% immediate after \begin{document}

% Setup old style numerals macro
\newcommand\osn[1]{\oldstylenums{#1}\xspace}

% Setup a definition style macro
\newcommand\defn[1]{\textbf{#1}}

